CAT: Compression-Aware Training for bandwidth reduction

Convolutional neural networks (CNNs) have become the dominant neural network architecture for solving visual processing tasks. One of the major obstacles hindering the ubiquitous use of CNNs for inference is their relatively high memory bandwidth requirements, which can be a main energy consumer and throughput bottleneck in hardware accelerators. Accordingly, an efficient feature map compression method can result in substantial performance gains. Inspired by quantization-aware training approaches, we propose a compression-aware training (CAT) method that involves training the model in a way that allows better compression of feature maps during inference. Our method trains the model to achieve low-entropy feature maps, which enables efficient compression at inference time using classical transform coding methods. CAT significantly improves the state-of-the-art results reported for quantization. For example, on ResNet-34 we achieve 73.1% accuracy (0.2% degradation from the baseline) with an average representation of only 1.79 bits per value. Reference implementation accompanies the paper at https://github.com/CAT-teams/CAT

==> sections/05_hardware.tex <==
\section{Hardware Implementation}
\label{sec:HW}
Our scheme doesn't require additional computational overhead over CNN basic layers. Hence, the total consuming energy can only be reduced.  The reduction ratio depends on hardware implementation details such as micro-architecture and the type of the processor and etc. 
For providing proof of concept of the energy consumption reduction on custom hardware, we implemented various convolutional layers that consist of common CNNs using in embedded systems such as ResNet and MobileNet. 
The hardware logic was designed using VHDL and Cadence Virtuoso for synthesis/place-and-route on a silicon die. We have used 65nm processor by TSMC. 

\CB{Add HW code to github}
\ez{details about Huffman?}


\begin{figure}
 \centering
 
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figures/energy_bars.pdf}
        \subcaption{ }
        \label{fig:energy}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \subcaption{\ez{accuracy vs.\ energy consumption for ResNet} }
        \label{fig:acc}
    \end{subfigure}
 \caption{}
        \label{fig:hardware}
\end{figure}
